Discrete Semantic Tokenization for Deep CTR Prediction

Incorporating item content information into click-through rate (CTR) prediction models remains a challenge, especially with the time and space constraints of industrial scenarios. The content-encoding paradigm, which integrates user and item encoders directly into CTR models, prioritizes space over time. In contrast, the embedding-based paradigm transforms item and user semantics into latent embeddings, subsequently caching them to optimize processing time at the expense of space. In this paper, we introduce a new semantic-token paradigm and propose a discrete semantic tokenization approach, namely UIST, for user and item representation. UIST facilitates swift training and inference while maintaining a conservative memory footprint. Specifically, UIST quantizes dense embedding vectors into discrete tokens with shorter lengths and employs a hierarchical mixture inference module to weigh the contribution of each user--item token pair. Our experimental results on news recommendation showcase the effectiveness and efficiency (about 200-fold space compression) of UIST for CTR prediction.

==> Review/www2024.comments-orig.tex <==
Review 1
Overall evaluation	
2: (accept)
This paper proposed an approach to CTR prediction / recommendation problem. It is well written overall and easy to follow. While the industry generally prefers embedding based models given its simplicity and effectiveness; the proposed method is worth exploring. While the MIND dataset is from real world data, the scale is still small in industry application standard. I would like to see the author expand more analysis on scaling up into real world situations like how to tackle the evolving item sets in recommendation list and added complexity in the training and inference architecture.

==> Review/www2024.comments.tex <==
# Review 1

1. While the MIND dataset is from real world data, the scale is still small in industry application standard. I would like to see the author expand more analysis on scaling up into real world situations like how to tackle the evolving item sets in recommendation list and added complexity in the training and inference architecture.

Qijiong: The MIND dataset, while not overly large, is sufficiently comprehensive to demonstrate the efficacy of our proposed method. Finding a dataset with item content of the same high quality, especially in the context of content-based recommendation, is challenging. Nonetheless, we acknowledge the value in testing our method on a larger-scale industrial dataset, which could further validate its robustness, even in scenarios like online learning where new data is continuously integrated. Due to the inaccessibility to such data and the limitation of our computational resources, we are unable to perform such extensive testing ourselves. However, we hope our work inspires industrial researchers to conduct their own evaluations.
